Stable Sparse Operator Inference for Nonlinear Structural Dynamics

Structural dynamics models with nonlinear stiffness appear, for example, when analyzing systems with nonlinear material behavior or undergoing large deformations. For complex systems, these models become too large for real-time applications or multi-query workflows. Hence, model reduction is needed. However, the mathematical operators of these models are often not available since, as is common in industry practice, the models are constructed using commercial simulation software. In this work, we propose an operator inference-based approach aimed at inferring, from data generated by the simulation model, reduced-order models (ROMs) of structural dynamics systems with stiffness terms represented by polynomials of arbitrary degree. To ensure physically meaningful models, we impose constraints on the inference such that the model is guaranteed to exhibit stability properties. Convexity of the optimization problem associated with the inference is maintained by applying a sum-of-squares relaxation to the polynomial term. To further reduce the size of the ROM and improve numerical conditioning of the inference, we also propose a novel clustering-based sparsification of the polynomial term. We validate the proposed method on several numerical examples, including a representative 3D Finite Element Model (FEM) of a steel piston rod.

==> creepmodel.tex <==
\subsection{Creep deformation}
Creep deformation is a widespread mechanical fatigue mode. It has a non-elastic characterization and occurs mostly due to high temperatures. However, the stresses do not cross the yield strength. Typically, the experiments allow to distinguish between three creep phases during the deformation.

\subsection{Lifted Creep Model}

Here we assume that for the change of the creep rate, the Garofalo creep law holds:

\begin{align} \label{eq:gar1}
    \dot{\varepsilon}_{\text{cr}} = C_1 (\sinh({C_2\sigma_v}))^n,
\end{align}
with $n \in \R. $ The ODE \eqref{eq:gar1} is scalar and $\varepsilon_{\text{cr}}$ stands for the effective (i.e. von Mises) creep strain. Note, that in practice, the Garofalo law describes the secondary creep state (i.e. steady-state creep).

The analog vector-form of the equation \eqref{eq:gar1} is given by
\begin{align} \label{creep}
    \dot{\Vec{\varepsilon}}_{\text{cr}} = C_1 (\sinh({C_2\sigma_v}))^n\frac{ \text{dev}(\Vec{\sigma})}{\sigma_v}.
\end{align}
In turn, the Cauchy stress is given by
\begin{align} \label{stress}
    \Vec{\sigma} = C \left(\frac{1}{2}(\nabla \Vec{d} + \nabla \Vec{d}^T)- \Vec{\varepsilon}_{\text{cr}}\right),
\end{align}
where $\Vec{d} \in \R^3$ stands for displacement vector.

In this work we utilize the vector notation
\begin{align}
    \Vec{\sigma} = (\sigma_{11}, \sigma_{22}, \sigma_{33}, \sigma_{12}, \sigma_{23}, \sigma_{13})^T, \     \Vec{\varepsilon}_{\text{cr}} = (\varepsilon^{\text{cr}}_{11}, \varepsilon^{\text{cr}}_{22},\varepsilon^{\text{cr}}_{33},\varepsilon^{\text{cr}}_{12}, \varepsilon^{\text{cr}}_{23}, \varepsilon^{\text{cr}}_{13})^T
\end{align}
The symmetrized gradient of the displacements is accordingly denoted as
\begin{align}
    \nabla_s\Vec{d} = \frac{1}{2}(\nabla \Vec{d} + \nabla \Vec{d}^T) \in \R^6.
\end{align}

We introduce the following (lifted) variable
%\begin{align}
%    \Vec{z} = (\Vec{z}_1, \Vec{z}_2, \Vec{z}_3, \Vec{z}_4, z_5, z_6, z_7, z_8)^T := \big(\Vec{d},\Vec{v}, \Vec{\varepsilon}_{\text{cr}},  \sinh^{n}({C_2\sigma_v}), \frac{e^{\sigma_v}}{2}, \frac{e^{-\sigma_v}}{2}, \frac{1}{\sinh({C_2\sigma_v})}, \frac{1}{2\sigma_v}\big)^T
%\end{align}

The von Mises stress in case of a three-dimensional stress is defined as
\begin{align}
\sigma_v = \sqrt{(\sigma_{11}-\sigma_{22})^2 + (\sigma_{22}-\sigma_{33})^2 + (\sigma_{33}-\sigma_{11})^2 + 3\sigma_{12}^2+ 3\sigma_{23}^2+ 3\sigma_{13}^2}
\end{align}
and hence
\begin{align}
    \dot{\sigma_v} = \frac{1}{2\sigma_v}\Vec{\sigma}^T\Vec{C}^{\sigma}\dot{\Vec{\sigma}}
\end{align}
with  $\Vec{C}^{\sigma} \in \R^{6 \times 6}$ given by
\begin{align}
    \Vec{C}^{\sigma} = \begin{pmatrix}
    2 & -1 & -1 &   &   &\\
    -1 & 2 & -1 &   &   &\\
    -1 & -1 & 2 &   &   &\\
       &    &   & 6 &   &\\
       &    &   &   & 6 &\\
       &    &   &   &   & 6
    \end{pmatrix}
\end{align}


Using the newly introduced notation we first consider \eqref{creep}, which turns into
\begin{align}
    \dot{\Vec{z}}_3 = C_1\Vec{z}_4 z_6 \text{dev}(\Vec{z_4}),
\end{align}
where $\text{dev}$ is a linear vector-valued function given by
\begin{align}
\text{dev}:
    \begin{pmatrix}
    z_1 \\
    z_2 \\
    z_3 \\
    z_4 \\
    z_5 \\
    z_6 \\
    \end{pmatrix} \mapsto
        \begin{pmatrix}
    z_1 - \gamma \\
    z_2 - \gamma \\
    z_3 - \gamma\\
    z_4 \\
    z_5 \\
    z_6 \\
    \end{pmatrix},\ \gamma = \frac{1}{3}(z_1+z_2 +z_3)
\end{align}
In addition, due to \eqref{stress}, the stress rate is given by
\begin{align}
    \dot{\Vec{\sigma}} &=  C \left(\frac{1}{2}(\nabla \Vec{v} + \nabla \Vec{v}^T)- \dot{\Vec{\varepsilon}}_{\text{cr}}\right)\\
    & =  C \left(\frac{1}{2}(\nabla \Vec{v} + \nabla \Vec{v}^T) - C_1 \sinh^n({C_2\sigma_v})\frac{\text{dev}(\Vec{\sigma})}{\sigma_v}\right)
\end{align}



Based on the lifting procedure from \cite{qian2020lift}, the governing equations
\begin{align}
        \dot{\Vec{d}} &= \Vec{v},\\
        \dot{\Vec{v}} &= \nabla \cdot C \left(\frac{1}{2}(\nabla \Vec{d} + \nabla \Vec{d}^T) - \Vec{\varepsilon}_{\text{cr}}\right) + \Vec{F},\\
        \dot{\Vec{\varepsilon}}_{\text{cr}} &= C_1 \sinh^n({C_2\sigma_v})\frac{\text{dev}(\Vec{\sigma})}{\sigma_v}
\end{align}
can be transformed into
\begin{align}
\dot{\Vec{z}}_1 &  =\Vec{z}_2 \\
\dot{\Vec{z}}_2 &= \nabla \cdot \Vec{C} (\nabla_s \Vec{z}_1 - \Vec{z}_3) + \Vec{F},\\
\dot{\Vec{z}}_3 &= 2C_1 z_4 z_8 \text{dev}(\Vec{C} ( \nabla_s \Vec{z}_1- \Vec{z}_3)),\\
\dot{z}_4  &= n C_2z_4z_7 z_8 (z_5+z_6)g(\Vec{z}_1,\Vec{z}_2, \Vec{z}_3, z_4, z_8 ),\\
\dot{z}_5 &=z_5z_8 g(\Vec{z}_1,\Vec{z}_2, \Vec{z}_3, z_4, z_8 )\\
\dot{z}_6 &= -z_6z_8 g(\Vec{z}_1,\Vec{z}_2, \Vec{z}_3, z_4, z_8 )\\
\dot{z}_7 &= - z_7^2 (z_5+z_6)g(\Vec{z}_1,\Vec{z}_2, \Vec{z}_3, z_4, z_8 ),\\
\dot{z}_8 &= -z^3_8 g(\Vec{z}_1,\Vec{z}_2, \Vec{z}_3, z_4, z_8 )
\end{align}
with 
%\begin{align}
%    g(\Vec{z}_1,\Vec{z}_2, \Vec{z}_3, z_4, z_8 ) = (\nabla_s\Vec{z}_1-\Vec{z}_3)^T\Vec{C}^T\Vec{C}^\sigma (\nabla_s \Vec{z}_2 - 2C_1 z_4 z_8 \text{dev}(\Vec{C} ( \nabla_s \Vec{z}_1- \Vec{z}_3)))
%\end{align}
\subsection{Remarks}

\begin{itemize}
    \item The stress and the creep strain are symmetric (each with 6 DOF)
    \item For the derivation of the stress rate, the exchangeability of time and spatial derivatives is assumed to hold.
    \item The right hand-side load $F$ should be discussed. It might include both the thermal and the mechanical forces.
\end{itemize}

==> draft.tex <==
Within the reduced space the semi-discretized form of our thermal-creep models is assumed as follows:
\begin{align}
    M_T\dot{T} + K_T T &= Q(t),\\
    M_u\ddot{u} + K_u u + f(t,u) &= F(t) - K_{Tu}T,
\end{align}
where $K_{Tu}$ is a constant coupling matrix between the temperature and displacements and $f(t,u)$ is the temperature-independent nonlinear part.

\begin{align}
    \ddot{u} + A_u u + A_{\text{cr}}\varepsilon^{\text{cr}} &= f_T\\
    \dot{\varepsilon^{\text{cr}}} &= ...\\
\end{align}
